Fast matrix-free methods for model-based personalized synthetic MR imaging

Synthetic Magnetic Resonance (MR) imaging predicts images at new design parameter settings from a few observed MR scans. Model-based methods, that use both the physical and statistical properties underlying the MR signal and its acquisition, can predict images at any setting from as few as three scans, allowing it to be used in individualized patient- and anatomy-specific contexts. However, the estimation problem in model-based synthetic MR imaging is ill-posed and so regularization, in the form of correlated Gaussian Markov Random Fields, is imposed on the voxel-wise spin-lattice relaxation time, spin-spin relaxation time and the proton density underlying the MR image. We develop theoretically sound but computationally practical matrix-free estimation methods for synthetic MR imaging. Our evaluations demonstrate superior performance of our methods in currently-used clinical settings when compared to existing model-based and deep learning methods. Moreover, unlike deep learning approaches, our fast methodology can synthesize needed images during patient visits, with good estimation and prediction accuracy and consistency. An added strength of our model-based approach, also developed and illustrated here, is the accurate estimation of standard errors of regional contrasts in the synthesized images. A R package $symr$ implements our methodology.

==> C-sim-old.tex <==
\section{Performance evaluations} % 3 pages 
\label{sec:sim}
\subsection{Experimental framework}
\label{sec:experiments}
Our AECM methodology was evaluated relative to LS and OSL-EM on 3D
magnitude MR images of a normal healthy male volunteer acquired
using the spin-echo imaging sequence at 12 (TE,TR)
settings~\citep{maitraandriddles10}. The datasets  were acquired on a
1.5T Signa scanner using spin-echo imaging sequence at a resolution of
$1.15 \text{mm}\times 1.15 \text{mm} \times 7.25 \text{mm}$ in a
field of view set to be $ 294 \text{mm}\times 294 \text{mm}\times
145 \text{mm}$. For each 3D image volume,  $n_x=n_y=256$ and
$n_z=20$. From the 12 images, we initially chose three images for our
training images and used the LS, OSL-EM and AECM algorithms to
estimate $\rho$, $\T_1$ and $\T_2$ at each voxel. These estimates were
then inserted into~\eqref{eq:bloch} along with design parameters
corresponding to the remaining nine images. The predicted synthetic
images were then compared to the acquired images to evaluate each of
the LS, OSL-EM and AECM methods. Our evaluations were done
visually as well as numerically.

For numerical measures, we used the root mean squared prediction error (RMSPE) for the $j$th image image volume, given by $\sqrt{\sum_{i=1}^n (r_{ij} - \widehat\nu_{ij})^2/n}$. We also calculated the mean
absolute prediction error (MAPE), defined for the $j$th image volume as
$ \sum_{i=1}^n |r_{ij} - \widehat\nu_{ij}|/n$.  In order to compare
across predicted images obtained at different settings, we scaled the
RMSPE by the standard deviation of the foreground voxel values in
$j$th acquired image. Similarly the MAPE was scaled by the mean
absolute deviation from the mean of the foreground voxels of the $j$th
acquired image.  
Finally, our evaluations calculated
$\widehat\nu_{ij}$ from the predicted $\nu_{ij}$ in two ways. First, we used
$\widehat\nu_{ij}$ without accounting for the Rice distribution
of the voxel-wise predictions. In the second case, we set $\widehat\nu_{ij}^* =
\hat\sigma_j\sqrt{\pi/2} 
\L_{1/2}\left(-{\hat{\nu}_{ij}^2/\hat{\sigma}_j^2}\right)$, or the mean
of the Rice distribution with parameters $\widehat\nu_{ij}$ and
$\hat\sigma_j$, with $ \L_{1/2}(x) =
e^{x/2}\left[\left(1-x\right)\I_{0}\left(-{x/2}\right)-x\I_{1}\left(-{x/2}\right)\right]$ denoting the Laguerre polynomial of order $1/2$. 

\subsection{Results}
We now discuss results of our experiments, 
all done using parallel computations on a 2.3GHz Intel(R) Xeon(R) Gold
6140 processor, capable of handling up to 36 threads.
\subsubsection{Illustrative performance of AECM}
\label{sec:ill}
We first illustrate performance of our AECM  on three training images
with $(\TE,\TR)\!\in\!\{ (10,0.6), (80,2), (10,3)\}$, here, TE times are in
milliseconds and  TR times in seconds. The three training images are
displayed in Figure~\ref{fig:3dplots_train}.

\begin{figure}
  \vspace{-0.1in}
	\centering
	\subfloat{\includegraphics[width=\linewidth]{figures/train_3D_plot_zlim_1}} \vspace*{-0.9em}
    \subfloat{\includegraphics[width=\linewidth]{figures/train_3D_plot_zlim_2}} \vspace*{-0.9em}
	\subfloat{\includegraphics[width=\linewidth]{figures/train_3D_plot_zlim_3}} \vspace*{-0.15em}
	\caption{Mid-axial (top), mid-coronal (middle), and mid-sagittal (bottom) views of training images with (from left to right) $\TE/\TR =10/600, 80/2000, 10/3000$ (in milliseconds).}  
	\label{fig:3dplots_train}
\end{figure}
% \printinunitsof{in}\prntlen{\textwidth} %7.1413 
% \printinunitsof{in}\prntlen{\linewidth} %3.48761 
% \printinunitsof{in}\prntlen{\textheight} %9.63245

Figure~\ref{fig:likeliplot} shows the objective function
in~\eqref{eq:penalizedproblem} as the OSL-EM and AECM algorithms 
proceed from LS initialization. In this example, OSL-EM is seen to
have an uncertain trajectory, and on the whole, actually goes down. On
the other hand, AECM correctly increases and terminates in a few
iterations. Our implementation of AECM ensures that this accuracy does 
not come at a price, with estimation and synthetic image generation
having in seconds. We now discuss performance.

\begin{figure}  
 \vspace{-0.1in}
  \centering
%  \mbox{
    \subfloat{
        \includegraphics[width=\linewidth]{figures/3D_plots_case_2_zlim_1.pdf}
      } 
%  } 
  \vspace*{-0.8em}
%   \mbox{
    \subfloat{
      \includegraphics[width=\linewidth]{figures/3D_plots_case_2_zlim_2.pdf}
    }
%   } 
  \vspace*{-0.8em}
%  \mbox{
    \subfloat{
      \includegraphics[width=\linewidth]{figures/3D_plots_case_2_zlim_3.pdf}
%    }
    \vspace*{-0.1in}
  }
  \vspace{-0.1in}
  \mbox{\subfloat{\includegraphics[width=0.5\linewidth]{figures/palette-crop.pdf}}}
	\caption{Mid-axial (top block), mid-coronal (middle), and
          mid-sagittal (bottom block) of the test images. In each
          block, the top row displays the observed test images, the
          second row displays the AECM-generated synthetic images
          $\widehat\nu$, and the bottom row displays the improvement
          in performance of the AECM over LS in predicting the test
          images for the best, the median and the worst performer among the test images. 
%          difference of $|\text{AECM} - \text{test images}| -
%          |\text{Least square} - \text{test images}|$ for each views
%          with scaling corresponding to the function
%          $\text{sgn}(x)\log(1+|x|).$
        }
	\label{fig:3dplots_all_mu}
\end{figure}
Figure~\ref{fig:3dplots_all_mu} and Table~\ref{table:3D_best} display performance of AECM on generating synthetic MR images at the test
design parameter settings. The figures indicate fairly accurate
reproduction of the test images by the AECM-estimated synthetic
images. This is further vindicated by Table~\ref{table:3D_best}.
\begin{table}[h!]
	\centering
	\caption{The 12 TE (in milliseconds), TR (in seconds) settings
          along with scaled root mean square prediction error (RMSPE),
          scaled mean absolute prediction error (MAPE) from the
          best training set (scale: $\times 0.01$).}% Prediction measures are calculated using $\nu^*$ as the $\widehat\nu$ and the mean of the corresponding Rice distribution}
	\label{table:3D_best}
	%\begin{spacing}{0.9}
        \centering
        \resizebox{0.5\textwidth}{!}{
		%\small
			\begin{tabular}{p{1mm}rp{3.75mm}|rr|rr}
				\hline
				\multicolumn{3}{c|}{Settings} & \multicolumn{2}{|c}{RMSPE} & \multicolumn{2}{|c}{MAPE} \\ 
				\hline
				j & TE & TR & $\widehat\nu$ & $\widehat\nu^*$ & $\widehat\nu$ & $\widehat\nu^*$ \\
				\hline
				\rowcolor{SkyBlue}
				1 & 10 & 0.6  & 3.23 & 3.22 & 6.94 & 6.96 \\ 
				2 & 15 & 0.6  & 13.65 & 13.66 & 15.71 & 15.72 \\ 
				3 & 20 & 0.6  & 15.94 & 15.97 & 18.12 & 18.15 \\ 
				4 & 10 & 1.0 & 16.90 & 16.89 & 21.02 & 21.01 \\ 
				5 & 30 & 1.0 & 19.22 & 19.24 & 22.28 & 22.30 \\
				6 & 40 & 1.0&21.20 & 21.22 & 24.04 & 24.06 \\ 
				7 & 10 & 2.0&33.65 & 33.62 & 43.85 & 43.81 \\ 
				8 & 40 & 2.0& 18.78 & 18.78 & 21.55 & 21.56  \\ 
				\rowcolor{SkyBlue}
				9 & 80 & 2.0& 1.14 & 1.15 & 4.94 & 4.94  \\ 
				\rowcolor{SkyBlue}
				10 & 10 & 3.0& 1.74 & 1.75 & 3.52 & 3.55  \\
				11 & 60 & 3.0&20.73 & 20.72 & 24.14 & 24.13 \\  
				12 & 100 & 3.0&28.29 & 28.21 & 33.32 & 33.26 \\ 
				\hline
			\end{tabular}
		}
	%\end{spacing}
\end{table}
Figure~\ref{fig:3dplots_all_mu} also displays
the voxel-wise difference in the absolute deviation of the AECM
predictions from the test images, and the LS predictions from the test
images, and shows overall improvement. (The overall numerical improvement of
AECM over LS in this example is quantified a little later in
Table~\ref{table:3D_best_10_whole_v2}.)  

\subsubsection{Choice of Optimal Training Set}
Following~\citep{maitraandriddles10}, we also investigate all possible
$(\TE, \TR)$ settings to see if some $(\TE, \TR)$ settings
provide better synthetic images. There are ${}^{12}C_{3}=220$
possible sets of three training images, but some of them are not
distinct, so they are discarded, leaving behind 212 sets.
For each set of three training images, we obtained LS, OSL-EM and
AECM-estimated parameters and then obtained synthetic images for the
nine $(\TE, \TR)$-values outside the considered training set. Table~\ref{table:3D_best_10_whole_AECM}
\begin{table}[h!]
	\caption{The  ten best sets of three training images and their performance (scale: $\times0.01$).} 
	\label{table:3D_best_10_whole_AECM}
	\centering
        \vspace{-0.05in}
	%\begin{singlespace}
	%\begin{spacing}{1.1}
		{\footnotesize 
			%\resizebox{1\textwidth}{!}{
				\begin{tabular}{r|r|r|r|r}
                \hline
                 Training & \multicolumn{2}{|c}{RMSPE} & \multicolumn{2}{|c}{MAPE} \\ 
                 \cmidrule{2-5}
                 Images & $\widehat\nu$ & $\widehat\nu^*$ & $\widehat\nu$ & $\widehat\nu^*$ \\ 
                 \hline
                    1, 9, 10 & 20.927 & 20.924 & 24.891 & 24.889 \\ 
                    2, 9, 10 & 21.112 & 21.097 & 25.081 & 25.068 \\ 
                    2, 10, 12 & 21.599 & 21.597 & 25.706 & 25.704 \\ 
                    2, 7, 9 & 21.383 & 21.349 & 25.340 & 25.324 \\ 
                    1, 10, 12 & 21.637 & 21.642 & 25.767 & 25.774 \\ 
                    1, 7, 9 & 21.536 & 21.539 & 25.537 & 25.541 \\ 
                    1, 8, 9 & 21.542 & 21.528 & 24.974 & 24.964 \\ 
                    1, 10, 11 & 21.856 & 21.833 & 25.825 & 25.808 \\ 
                    2, 10, 11 & 21.913 & 21.885 & 25.887 & 25.864 \\ 
                    2, 8, 9 & 21.602 & 21.586 & 25.048 & 25.035 \\ 
                    \hline
                    \end{tabular}
			%}
		}
		%\end{singlespace}
	%\end{spacing}
\end{table}
 % Among these cases, we consider RMSPE and MAPE with two different $\widehat\nu_{ij}^*$ as discussed before and SSIM as our performance measures. The results are presented in \ref{table:3D_best_10_whole_v2}. It is ordered according to the increasing average RMSPE, which is not maintained for other measures, but these values show more or less consistent behavior. 
\begin{table*}[!h]
    \vspace*{-0.65em}
	\caption{The ten best training sets and their average
          performance measures relative to the LS estimates ($\times 0.01$).} 
	\label{table:3D_best_10_whole_v2}
	\centering
	%\begin{singlespace}
	%\begin{spacing}{1.1}
		{\footnotesize 
			%\resizebox{0.5\textwidth}{!}{
				\begin{tabular}{c|r|r|r|r|r|r|r|r}
                    \hline
                    & \multicolumn{4}{|c}{RMSPE} & \multicolumn{4}{|c}{MAPE}\\
                    \cmidrule{2-9}
                    Training & \multicolumn{2}{|c}{$\widehat\nu$} & \multicolumn{2}{|c}{$\widehat\nu^*$} & \multicolumn{2}{|c}{$\widehat\nu$} & \multicolumn{2}{|c}{$\widehat\nu^*$}
                    \\
                    \cmidrule{2-9}
                    Images & OSL & AECM & OSL & AECM & OSL & AECM & OSL & AECM \\
                    \hline
                    1, 9, 10 & -0.442 & 1.103 & -0.338 & 1.979 & -0.263 & 1.279 & 0.007 & 1.199  \\ 
                    2, 9, 10  & -0.643 & 1.276 & -0.504 & 2.413 & -0.471 & 1.489 & -0.089 & 1.443 \\ 
                    2, 10, 12 & -1.186 & 0.947 & -1.543 & 1.762 & -1.210 & 0.998 & -0.801 & 0.953  \\ 
                    2, 7, 9 & 0.678 & 3.415 & 1.530 & 6.552 & 1.225 & 3.506 & 1.321 & 3.439 \\ 
                    1, 10, 12 & -0.896 & 1.119 & -1.264 & 1.920 & -1.092 & 1.150 & -0.806 & 1.028  \\ 
                    1, 7, 9 & 0.137 & 2.967 & 0.774 & 5.780 & 0.645 & 2.960 & 0.871 & 2.938 \\ 
                    1, 8, 9 & 0.187 & 3.813 & 0.851 & 7.363 & -0.124 & 3.463 & 0.097 & 3.414 \\ 
                    1, 10, 11 & 0.021 & 1.047 & 0.566 & 2.008 & 0.148 & 1.084 & 0.358 & 1.049 \\ 
                    2, 10, 11 & -0.205 & 1.274 & 0.262 & 2.439 & -0.131 & 1.433 & 0.194 & 1.396 \\
                    2, 8, 9 & -0.004 & 3.242 & 0.594 & 6.351 & -0.382 & 3.028 & -0.090 & 3.022  \\ 
                    \hline
                \end{tabular}
			}
%		}
		%\end{singlespace}
	%\end{spacing}
\end{table*}
displays numerical performance of the AECM-estimated synthetic images for the top 10 combinations (ordered according to the increasing scaled RMSPE). Table~\ref{table:3D_best_10_whole_v2}
shows the per cent improvement of AECM and OSL-EM over LS for each of
the measures. We see around 5\% improvement of AECM over LS. Once
again, OSL-EM is unpredictable in its improvement over LS, often doing worse. 
\subsubsection{Consistency}
A desirable feature of any estimation or prediction method is
statistical consistency, or improvement in performance as more
information (training image set) becomes available. Therefore, we
considered and evaluated performance of the AECM method in generating
synthetic images as the number of images in the training set increased
over $m\in\{3, 4, 5,\dots, 11\}$. For each $m$, we evaluated
predictive performance with a training set of images of all possible training image set combinations of size $m$ and compared them with the remaining images in the test sample. The RMSPE and MAPE
values for the best set, and for each $m$ are displayed in
Figure~\ref{fig:3D_consistency} and show consistency of our synthetic
image generation method. 
\begin{figure}[!t]
	\centering
    \includegraphics[width=\linewidth]{figures/Consistency-5-crop.pdf}
	\caption{The best training samples for varying training sample
          sizes and their performance measures.}
	\label{fig:3D_consistency}
\end{figure}
% \begin{table*}[!htb]
% 	\caption{The best training samples for varying training sample sizes and the corresponding performance measures (average RMSPE ans SSIM, in \%) for the 3D MR dataset.} 
% 	\label{table:3D_consistency}
% 	\centering
% 	%{\footnotesize
% 	%\resizebox{0.5\textwidth}{!}{
% 		\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
% 			\hline
% 			m & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 \\ 
% 			\hline
% 			Best Avg. RMSPE & 11.19 & 10.84 & 9.72 & 9.26 & 8.74 & 8.26 & 8.04 & 7.70 & 7.85 \\ 
% 			Best SSIM & 98.371 & 98.699 & 99.019 & 99.129 & 99.271 & 99.316 & 99.380 & 99.422 & 99.469 \\ 
% 			\hline
% 		\end{tabular}
% 	%}
% 	%}
% \end{table*}
%% Another way of dealing this part would be through a figure so that
%% two column would not be wasted and the next image fits better??  We can see, in general, in terms of best Average RMSPE and best SSIM, the performance measure is gets better as the number of training sample increases, representing consistency of our method. 
% \begin{comment}
% \subsection{2D Phantom Dataset}
% The 2D data sets were acquired on a 1.5T sigma scanner using a spin-echo imaging sequence with the dimension $256 \times 256$. 
% % Was it more powerful?
% For this data also, we follow similar procedures to train and test. The predictive performances are better than the 3D case in general. The choice of best train set is chosen as before and again this time. 
% The TE, TR values of the best set are: $(60, 1000), (30, 2000), (80, 3000)$, which may be identified as $\T_1, \rho, \T_2$-weighted images. 
% The performance measures are as in table \ref{table:2D_best_10_whole_v2}. 
% \begin{table*}[h!]
% 	\caption{The best 10 training samples and the corresponding performance measures for the 2D phantom dataset - version 2.} 
% 	\label{table:2D_best_10_whole_v2}
% 	\centering
% 	%\begin{singlespace}
% 	\begin{spacing}{1.0}
% 		{\footnotesize 
% 			\resizebox{1\textwidth}{!}{
% 				\begin{tabular}{p{0.1cm}l|cccccccccc}
% 					%\cline{3-12}
% 					%& & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
% 					\cmidrule{1-12}
% 					& Train Ind. & 2, 7, 16 & 1, 10, 15 & 1, 10, 17 & 3, 10, 17 	& 3, 10, 13 & 5, 10, 15  & 5, 10, 13 & 3, 12, 13 & 5, 12, 13 & 1, 12, 15 \\ 
% 					\midrule
% 					\midrule
% 					\multirow{3}{*}{\rotatebox[origin=c]{90}{LS}} 
% 					& Avg. RMSPE & 0.03280 & 0.03238 & 0.03269 & 0.03274 & 0.03273 & 0.03276 & 0.03343 & 0.03347 & 0.03388 & 0.03407 \\ 
% 					& Avg. MAPE & 0.04276 & 0.04114 & 0.04144 & 0.04123 & 0.04209 & 0.04150 & 0.04372 & 0.04206 & 0.04289 & 0.04227 \\ 
% 					& SSIM & 0.99885 & 0.99887 & 0.99890 & 0.99895 & 0.99884 & 0.99894 & 0.99879 & 0.99899 & 0.99899 & 0.99892 \\
% 					\midrule
% 					\multirow{3}{*}{\rotatebox[origin=c]{90}{OSL EM}} 
% 					& Avg. RMSPE & 0.03243 & 0.03245 & 0.03269 & 0.03279 & 0.03278 & 0.03284 & 0.03315 & 0.03341 & 0.03371 & 0.03411 \\
% 					& Avg. MAPE & 0.04115 & 0.04104 & 0.04161 & 0.04146 & 0.04164 & 0.04125 & 0.04207 & 0.04135 & 0.04190 & 0.04218 \\ 
% 					& SSIM & 0.99896 & 0.99889 & 0.99891 & 0.99897 & 0.99887 & 0.99896 & 0.99888 & 0.99903 & 0.99905 & 0.99894 \\
% 					\midrule
% 					\multirow{3}{*}{\rotatebox[origin=c]{90}{AECM}}
% 					& Avg. RMSPE & 0.03243 & 0.03245 & 0.03267 & 0.03275 & 0.03278 & 0.03283 & 0.03315 & 0.03341 & 0.03371 & 0.03411 \\ 
% 					& Avg. MAPE & 0.04114 & 0.04104 & 0.04159 & 0.04134 & 0.04164 & 0.04124 & 0.04206 & 0.04134 & 0.04190 & 0.04218 \\ 
% 					& SSIM & 0.99896 & 0.99889 & 0.99891 & 0.99897 & 0.99887 & 0.99896 & 0.99888 & 0.99903 & 0.99905 & 0.99894 \\ 
% 					\midrule
% 				\end{tabular}
% 			}
% 		}
% 		%\end{singlespace}
% 	\end{spacing}
% \end{table*}
% We only present the figures with the minimum, the median, and the maximum SSIM(0.9961241, 0.9995651, 0.9997736 respectively) for the 2D case from the 15 test case in the following figure \ref{fig:2dplots}, where the train images are the best combination of train images from the previous table: 
% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=0.8\linewidth, height=0.15\textheight, page=1]{image/2D_plots_case.pdf}
% 	\caption{3 among 15 2D phantom MR test images and corresponding predicted images using AECM; Top sub-row displays the observed images while the bottom sub-row displays the corresponding MPLE predicted images for all views. The images correspond to the minimum, median and the maximum SSIM respectively among 15 test images.}
% 	\label{fig:2dplots}
% \end{figure}

% The best performances for increasing training size is represented in table \ref{table:2D_consistency}: 
% \begin{table}[h!]
% 	\caption{The best training samples for varying training sample sizes and the corresponding performance measure(average RMSPE) for the 2D phantom dataset.} 
% 	\label{table:2D_consistency}
% 	\centering
% 	{\footnotesize
% 		\resizebox{1.025\textwidth}{!}{
% 			\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% 				\hline
% 				m & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 \\ 
% 				\hline
% 				Avg. RMSPE & .0324 & .0291 & .0286 & .0269 & .0276 & .0262 & .0258 & .0252 & .2500 & .0243 & .0237 & .0229 & 0.0226 & 0.0214 & 0.0199 \\ 
% 			\hline
% 			\end{tabular}
% 		}
% 	}
% \end{table}
% \end{comment}
%\subsection{Convergence Trajectories and CPU times}
%As discussed in the previous section, OSL-EM addresses the same modeling approach, but with a different numerical method, which does not guarantee the ascending of EM algorithm. A more elaborate illustrative example is discussed in Section \ref{sec:supp-trajectory-likeli}. Also, our AECM method does predict Synthetic-MR images in real-time, even without the numerical changes as applied in OSL-EM. If the initial value for the algorithm is taken from the LS estimate for both AECM and OSL, the consumed time is comparable as discussed in Section~\ref{sec:supp-time-comparison}. 
% We also have the SSIM values over different dimensions represented as violin plots in \ref{fig:SSIM}. 
% \begin{figure}[!h]
% 	\centering
% 	\includegraphics[width=\linewidth]{image/SSIM_dims.pdf}
% 	\caption{violin plots of SSIM values over different dimensions for the test part of 3D dataset, trained with the best image set}
% 	\label{fig:SSIM}
% \end{figure}
% \begin{figure*}[!h]
% 	\centering
% 	\begin{subfloat}[b]{\textwidth}
% 		\includegraphics[width=1\linewidth]{image/new/All_zlim_1.pdf}
% 		\caption{}
% 		\label{fig:3D1all} 
% 	\end{subfloat}
	
% 	\begin{subfloat}[b]{\textwidth}
% 		\includegraphics[width=1\linewidth]{image/new/All_zlim_2.pdf}
% 		\caption{}
% 		\label{fig:3D2all}
% 	\end{subfloat}
	
% 	\begin{subfloat}[b]{\textwidth}
% 		\includegraphics[width=1\linewidth]{image/new/All_zlim_3.pdf}
% 		\caption{}
% 		\label{fig:3D3all}
% 	\end{subfloat}
% 	\caption{Mid-axial \ref{fig:3D1all} Mid-coronal \ref{fig:3D2all} and Mid-sagittal \ref{fig:3D3all} views; Top row displays the observed images, 2nd row displays the AECM estimate, while the next rows displays the difference corresponding to the Least Square Algorithm, OSL algorithm and AECM algorithm.}
% 	\label{fig:3dplotsall}
% \end{figure*}
\subsection{Estimating SEs of ROI means}
Our final set of evaluations is on estimating SEs of ROI means in
synthetic images obtained using the training set in
Figure~\ref{fig:3dplots_train}. We considered three ROIs consisting of 
Cerebro-Spinal Fluid (CSF), Gray Matter (GM) and White Matter
(WM). Table~\ref{table:variance} provides the ROI means of the
synthetically generated variances. The machinery of
Section~\ref{variance} was used to estimate SEs of the ROI means
and compared with computationally expensive boostrap
estimates. %obtained using computationally expensive 200 bootstrap replications. 
% For each synthetic image, we calculated the mean values of the s We have estimated the variances of a linear combination of voxels using the information matrix and parametric bootstrap for the test images. The vector corresponding to the linear combination corresponds to a scaled version of the indicators of Cerebro-Spinal Fluid (CSF), Gray Matter (GM) and White Matter (WM), respectively, such that their sum is $1$. Both the methods give comparable results as seen in table~\ref{table:variance}. 
%The tolerance used in the Lanczos algorithm was set to $10^{-6}$. Also, we fixed the maximum iteration to $1000$ for this algorithm. For the parametric bootstrap, we have used $200$, resampled images. For all the estimations in the parametric bootstrap, the conditions were the same as the original estimations. 
(For details, see Section~\ref{sec:supp-para-boot}, which also shows
insignificant differences between our estimates and the bootstrap-estimated SEs.) 
% A jackknife-type method was used to estimate the variability in the
% boottrap We have also applied a Jackknife-type variance estimator
% for the parametric bootstrap-based estimates of SE of the linear
% combinations. For all the tissue types and test images, the SE of
% the linear combination estimated by the Information matrix falls
% inside twice the SE of the Parametric bootstrap SE estimate. Also,
% visually, we can see that those are relatively close to each other.  
\begin{table}
	\centering
	\caption{Estimated CSF, GM and WM ROI means in synthetic
          images and their SEs: $\widehat\sigma_s$s calculated using
          the formula in Section~\ref{variance}, and
          $\widehat\sigma_b$s estimated using parametric
          bootstrap. The scale for the SEs is $\times10^{-3}$.} 
	\label{table:variance}
	\resizebox{0.5\textwidth}{!}{
	    \begin{tabular}{c|rcc|rcc|rcc}
			    \hline 
			    \text{Image}  & \multicolumn{3}{c|}{\text{CSF}} & \multicolumn{3}{c|}{\text{GM}} & 
			    \multicolumn{3}{c}{\text{WM}} 
				\\
				\cmidrule{2-10}
				\text{$j$ } &  Mean & $\widehat\sigma_s$ & $\widehat\sigma_b$ &  Mean & $\widehat\sigma_s$ & $\widehat\sigma_b$ 
				&  Mean & $\widehat\sigma_s$ & $\widehat\sigma_b$\\
				\hline
				2 & 36.7 & 3.73 & 4.45 & 73.1 & 3.31 & 3.71 & 123.4 & 7.53 & 6.93\\ 
				3 & 33.8 & 3.95 & 4.15 & 67.9 & 3.05 & 3.41 & 111.4 & 7.07 & 6.61 \\ 
                4 & 57.7 & 5.11 & 5.62 & 112.7 & 4.09 & 4.62 & 167.1 & 7.73 & 7.38 \\ 
                5 & 42.0 & 4.13 & 4.35 & 84.0 & 2.99 & 3.28 & 110.5 & 6.22 & 6.07 \\ 
                6 & 36.3 & 3.85 & 4.07 & 72.8 & 2.74 & 2.95 & 90.0 & 6.44 & 6.52 \\ 
                7 & 88.4 & 5.55 & 5.70 & 164.0 & 3.96 & 4.23 & 191.4 & 9.86 & 9.52 \\ 
                8 & 55.9 & 4.44 & 4.51 & 106.4 & 2.79 & 2.77 & 102.7 & 7.21 & 7.24 \\ 
                11 & 52.6 & 5.42 & 5.41 & 93.4 & 3.59 & 3.73 & 69.8 & 7.44 & 7.80 \\ 
                12 & 33.3 & 5.13 & 4.69 & 54.5 & 3.39 & 3.49 & 31.1 & 5.74 & 6.18 \\ 
			\hline
		\end{tabular}
	}
\end{table}
% \begin{table}[ht]
% \centering
% \caption{Estimates Standard errors of parametric Bootstrap based SE of the corresponding linear combinations for three different tissue types}
% \label{table:se_of_se}
% \begin{tabular}{cccc}
%   \hline
%  & CSF & GM & WM \\ 
%   \hline
%   2 & 0.229 & 0.168 & 0.341 \\ 
%   3 & 0.221 & 0.155 & 0.317 \\ 
%   4 & 0.315 & 0.217 & 0.390 \\ 
%   5 & 0.278 & 0.159 & 0.291 \\ 
%   6 & 0.259 & 0.144 & 0.295 \\ 
%   7 & 0.294 & 0.210 & 0.541 \\ 
%   8 & 0.255 & 0.137 & 0.373 \\ 
%   11 & 0.245 & 0.159 & 0.373 \\ 
%   12 & 0.215 & 0.148 & 0.275 \\ 
%   \hline
% \end{tabular}
% \end{table}


==> introduction.tex <==
\newcommand{\TR}{{\textrm{TR}}}
\newcommand{\TE}{{\textrm{TE}}}
\newcommand{\T}{{\textrm{T}}}

\section{Introduction} %1 pages
\label{sec:intro}
\IEEEPARstart{M}{agnetic} Resonance~(MR) Imaging (MRI)~\citep{katims82,
  mansfieldandmorris82,hinshawandlent83} is a popular %has, over the
                                %past several decades, gained in
                                %popularity as a
radiologic tool for visualizing tissue structure or for characterizing
cerebral and other functions.  In MR imaging, each tissue type
has a distinctive  spin-lattice 
or longitudinal  relaxation time ($\T_1$), spin-spin or transverse
relaxation time ($\T_2$), and proton density ($\rho$). %In many MRI
% techniques,
These quantities are observed only indirectly through  
noise-contaminated measurements of their transformations that
moduldate their effect through user-controlled design parameters such as
echo time (TE), repetition time (TR) or flip angle ($\alpha$). Even when such images can be directly obtained, they are practically
unusable owing to their low resolution~\citep{deonietal05} or
acquisition times~\citep{warntjesetal08}. 

There are many ways~\citep{kuperman00,bernsteinetal04,brownetal14} in
which $\rho$, $\T_1$ and $\T_2$ combine with the design parameters to
form an MR image. In the specific illustrative case of
spin-echo MRI used in this paper, % for its convenience and
% simplicity,
the noiseless MR intensity ($\nu_{ij}$) (assuming perfect
excitation) at the $i$th voxel
and for the $j$th design parameter setting of TE and TR 
({\em i.e.}  with $(\mbox{TE}_j, \mbox{TR}_j)$) is approximately
specified by the Bloch equation
\begin{equation}
	\nu_{ij} = \rho_i \exp\left(-\frac{\TE_j}{\T_{2i}}\right)\left\{1 -
	\exp\left(-\frac{\TR_j}{\T_{1i}}\right)\right\}.
	\label{eq:bloch}
\end{equation}
\citet{maitraandriddles10} predicate~\eqref{eq:bloch} under the simplifying assumptions of a single perfect
$\alpha = 90^{\circ}$ relaxation pulse followed by a recovery time of length
$\TR_j$ and a delay of time $\TE_j$  for acquisition, and that
$\nu_{ij}$ is determined entirely by $\rho_i$, $\T_{1,i}$ and
$\T_{2,i}$ and is affected negligibly by other contrasts. In reality,
of course, the observed MR signal is noise-contaminated and 
complex-valued because it is acquired after Fourier reconstruction on
a Cartesian grid in $K$-space. The magnitude ($r_{ij}$, at the $i$th
voxel and $j$th design parameter setting) of this
complex-valued signal is commonly used, and is well-modeled~\citep{henkelman85, 
  sijbers98, sijbersetal98} by a Rice distribution~\citep{rice44, rice45} with density
\begin{equation}
	\varrho(r_{ij}; \sigma_j, \nu_{ij}) = \frac{r_{ij}}{\sigma_j^2} \exp\left(-\frac{r_{ij}^2 + \nu_{ij}^2}{2\sigma_j^2}\right)
	\I_0\left(\frac{r_{ij}\nu_{ij}}{\sigma_j^2}\right),
	\label{eq:rice}
\end{equation}
for $r_{ij}>0$. Here $\sigma>0$ is the scale parameter of the Rice
density and $\I_k(\cdot)$ is the modified Bessel function of the first
kind of order $k$. The Rice distribution of $r_{ij}$ follows from the
approximate distribution~\citep{wangandlei94} of the complex-valued MR signal as
bivariate Gaussian with mean $(\nu_{ij}\cos\eta,\nu_{ij}\sin\eta)$ and homogeneous diagonal dispersion matrix $\sigma^2\bI_2$, for some $\eta$. For identifiability and convenience,  we use $\eta=0$~\citep{maitraandfaden09,maitraandriddles10,maitra13}.

For a spin-echo MR imaging sequence~\citep{hahn50, hennigetal86},
different $(\TE,\TR)$ values modulate $\T_1$, $\T_2$ and $\rho$
and can be used to enhance the clinical distinction between tissues. 
% More specifically, $\T_1$, $\T_2$ are the times (or equivalently, their inverses $R_1, R_2$, the rates) to return to its equilibrium state after excitation by magnetization in the corresponding direction as the static magnetic field for the specific tissue-molecule. 
%These values are directly unobservable and practically unusable for many MR imaging methods. 
%Instead, we control scanner parameters, e.g., echo time (TE), repetition time (TR) or flip angle ($\alpha$) to control the influence of $\rho, \T_1, \T_2$ in an image. 
%The spin-echo image is acquired within a short span to provide high-resolution images with a high signal-to-noise ratio (SNR) but mixed contrasts(remove this sentence?). 
However, the optimal $(\TE, \TR)$-settings are patient- and/or
anatomy-specific and not always possible to specify in advance.
%This aspect is not specific to the spin-echo sequence but holds for
%other techniques also.
Patient discomfort, such as with children or claustrophobic
subjects, may, for example, preclude obtaining images with long
acquisition times. This phenomenon is by no means limited to the
spin-echo technique: for instance,  it is not possible to gather
$\T_1$ or $\T_2$  images using spoiled gradient recalled-echo (SPGR) or 
fully balanced  steady-state free precision (SSFP)
techniques, respectively~\citep{deonietal05}. Nevertheless,  
$\T_1$ and $\T_2$ images can, for instance, help distinguish
neurologically diseased
brains~\citep{larssonetal89,williamsonetal92,pitkanenetal96,vymazaletal99,bartzokisetal00,friedmanetal03}
and so may be important to acquire.

{\em Synthetic MRI} was proposed~\citep{bobmanetal85,
  bobmanetal86, feinbergetal85, ortendahletal84b,gonccalvesetal18} to address the above
shortcomings. In traditional synthetic MRI, the objective is to first
estimate the underlying $\rho,\T_1,$ and $\T_2$ values at a voxel from 
a set of {\em training} images and to insert these estimates along
with unobserved design parameters into~\eqref{eq:bloch}, in spin-echo
MRI, to obtain corresponding synthetic images. The technique is an
appealing alternative 
% potentially faster and less time-consuming alternative
in scenarios where images at  multiple settings are required, such as
in pediatric imaging of the developing brain or non-cooperating
subjects~\citep{bettsetal16, mcallisteretal17, andicaetal19}, or in patients
with multiple sclerosis~\citep{hagiwaraetal17b} and so on. In such
situations,  images with longer acquisition times can potentially be
synthesized from those collected with shorter acquisition times. 
Another benefit is a potential reduction in motion artifacts, or the
possibility of consistent image comparisons between different
settings. % as we have an approach of absolute                     % quantification of $\rho, \T_1, \T_2$ 
%In general, the spin-echo MR sequence can be broadly categorized into three classes: $\T1$-weighted images using a short TE, TR (a high signal for fat and paramagnetic materials); $\T2$-weighted using a long TE, TR (a high signal for water content, as in tumor, edema, hemorrhage); and $\rho$-weighted images with long TR and short TE (high signal from meniscus tears).
%Clinically, these volumetric $\T_1, \T_2$ mappings have shown promise in distinguishing neurologically diseased brains \citep{larssonetal89, bartzokisetal00, pitkanenetal96, williamsonetal92, friedmanetal03, vymazaletal99}. 
%For any specific voxel and a specific TE, TR settings, the machine captures noise-contaminated MR signals $r$, usually magnitude of a complex-valued Fourier reconstruction. This contaminated signal is well-modeled \citep{henkelman85, sijbers98, sijbersetal98} by a Rice distribution \citep{rice44, rice45}. 
%Under assumptions of a single perfect $90^{\circ}$ relaxation pulse followed by a recovery time of length $\TR$ and a $\TE$ time delay for acquisition, the noiseless signal $\nu$ is assumed to be related only to $\rho$, $\T_1$ and $\T_2$ (thus neglecting the effect of other contrasts). 
%At each voxel, $\nu$ is can be expressed as a solution to the Bloch equation, an empirically-derived set of differential equation describing nuclear magnetization \citep{hinshawandlent83}, in terms of $\T_1$, $\T_2$, and $\rho$. Specifically, the noiseless signal, $\nu$ is approximately given by $\displaystyle \rho \exp\left(-\TE/\T_{2}\right)\left\{1 - \exp\left(-\TR/\T_{1}\right)\right\}$ upto a proportionality constant. 
%Suppose we have a multiparametric MRI, i.e., a combination of more
%than one MR sequence of the same object and geometry but different
%TE, TR settings. The fundamentals of \emph{Synthetic Magnetic
%Resonance Imaging} \citep{bobmanetal85, bobmanetal86, feinbergetal85,
%ortendahletal84b} %% Include more -- the papers opened, include
%mainly from Hagiwara paper is to synthesize MR images with new design parameter (i.e., TE, TR) settings even when original images were not acquired in those exact settings. It is a potentially faster way than conventional MRI if images with different settings are required, which recently has been used in pediatrics for developing brain or non-cooperative patients \citep{bettsetal16, mcallisteretal17, andicaetal19}, multiple sclerosis \citep{hagiwaraetal17b}
%and other cases. Another advantage is the possibility of consistent image comparison between different settings. % as we have an approach of absolute quantification of $\rho, \T_1, \T_2$
%This equation is used to estimate the underlying $\rho, \T_1, \T_2$ for any voxel, and then the same equation~\eqref{eq:bloch} is used with desired TE, TR settings to generate the synthetic image. 
%The added advantage is obtaining images with longer acquisition times from less time-consuming images \citep{feinbergetal85} and also reduces the potential motion artifact.
However, despite its vast potential, synthetic MRI's clinical
adaptation has been stymied by the inherent ill-posedness of the
inversion of the Bloch equation. Because a handful of training images
are typically acquired, the standard voxel-wise least squares (LS) estimates of
$(\rho,\T_1,\T_2)$ are unstable \citep{maitraandriddles10}, leading to
the need for spatial regularization of these estimates. Bayesian
solutions~\citep{gladandsebastiani95,maitraandbesag98} imposed a
multi-layer extension of the Geman-McClure Markov random field 
prior \citep{gemanandmcclure93} on $(\rho,\T_1,\T_2).$ However, instead
of the Rice distribution \eqref{eq:rice}, they assumed $r_{ij}$ to be
independent Gaussian with mean $\nu_{ij}$ and variance $\sigma_j^2.$
In order to tackle the resulting intractability of the 
posterior distributions, \citet{gladandsebastiani95} resorted to a farrago of pseudo-likelihood, expectation-maximisation (EM) and Gibbs sampling while \citet{maitraandbesag98} used computationally intensive MCMC methods -- both of which are impractical to use on three-dimensional (3D) images in a clinical setting.

An alternative approach to synthetic MRI was proposed by
\citet{maitraandriddles10} who assumed more accurate Rice distributions
\eqref{eq:rice} for the $r_{ij}$'s and Gaussian Markov Random field
(GMRF) structure on transformations of ($\rho, \T_1, \T_2$). Although
they correctly anticipated that such a formulation of the synthetic
MRI problem should facilitate practically fast statistical
computations, their estimating algorithm, the one-step late EM (OSL-EM)
algorithm of \citet{green90}, is not guaranteed to converge, and can provide
suboptimal estimates % (see Figure \ref{fig:likeliplot})
when stricter convergence criteria are applied than in their paper. 

% who used penalized likelihood that
% incorporated the Rice distribution of the observed magnitude values at
% a voxel and a penalty that helped maintain spatial context through the
% use of an appropriate Matrix Normal prior distribution on a
% transformation of $\rho, \T_1, \T_2$. Implementation was through the 
% Expectation-Maximization(EM) algorithm~\citep{dempsteretal77}, however
% the penalty makes computations challenging so the One-Step-Late (OSL)
% EM (OSL-EM)~\citep{green90} was used even though this algorithm is not
% guaranteed to have the ascending property of the EM algorithm. 
% Instead, \cite{maitraandriddles10} consider the Rice distribution \eqref{eq:rice} but assume a multilayer intrinsic Markov random field prior on transformed $(\rho,T_1,T_2).$


% 
% The classical approach to performing synthetic MRI uses the
% method of least-squares (LS) to estimate the underlying $\rho$, $\T_1$
% and $\T_2$ images from those obtained at at least three (and rarely
% more) settings. Such an approach does not account for the
% ill-posedness of the inverse problem~\citep{osullivan86} that can
% yield unstable and spatially inconsistent esimates of 
% $\rho$, $\T_1$ and $\T_2$ at each voxel. As a result, the methodology
% had not been adopted much in clinical practice and radiologists have
% largely continued to base their diagnosis on two or three available
% images. For example, %In general, the spin-echo MR sequence can be
% % broadly categorized into three classes:
% it is common to acquire 
% $\T_1$-weighted images using a short TE and TR sequence (with high
% signal for fat and paramagnetic materials),  $\T_2$-weighted images
% using a long TE and TR sequence (with high signal for water content,
% as in tumor, edema or hemorrhage) or $\rho$-weighted images with a
% long TR and short TE sequence that has high signal from meniscus
% tears. However, such images, while useful in diagnosis, do not exploit
% the  full potential of MRI.  

% {\em To address these issues, \citet{warntjesetal08} used a modified LS
% approach. }
% \citet{gladandsebastiani95} and \citet{maitraandbesag98} proposed a
% Bayesian approach using an extended 
% Geman-McClure~\citep{gemanandmcclure93} Markov Random Field(MRF) prior
% on $\rho, \T_1, \T_2$ that accounts for spatial structure between
% their voxel-wise estimates.% which helps in alleviating the effects of
%                           % ill-posedness in the inversion of the
%                           % Bloch transform.
% However, estimation here requires the use of computationally
% expensive Markov Chain Monte Carlo(MCMC) methods that is impractical
% to use routinely or in clinical settings. Their 
% implementation uses an univariate Gaussian in lieu
% of the Rice distribution for the (magnitude of the) observed
% signal. While simplifying computations, such model mmisspecification
% can yield inaccurate estimates, especially in low-SNR situations.


% as regularization to the problem inducing corresponding MRF structures. They have used the Expectation-Maximization(EM) \citep{dempsteretal77} approach to maximize the penalized likelihood function with Rice distribution. More specifically, to computational efficiency, they have used a One-Step-Late (OSL) version of EM \citep{green90}, which hampered the guarantee of the ascending property of the EM algorithm. Moreover, even the OSL-EM estimation procedure was time-consuming \citep[Sec-III-B]{maitraandriddles10}. % See Section III-B - how to cite?

% For the estimation of $\rho, \T_1, \T_2$, we need at least three different settings MR image as we have three underlying parameters per voxel. The estimation can be done using the classical least square(LS) method \citep{blystadetal12, hagiwaraetal17a, gonccalvesetal18} - with possibly different approximations of the Bloch equations) corresponding to the Gaussian distribution, an approximation to Rice distribution. Nevertheless, the nature of the problem is ill-posed as the number of parameters is the same as the number of data-points. 

A machine learning approach~\citep{hagiwaraetal19} using
conditional generative 
adversarial networks (cGAN)~\citep{mirzaandosindero14} argued that 
$\T_1$ and $\T_2$-weighted images, generated by the LS-based SyMRI
software~\citep{hagiwaraetal17a} are of good quality, but that the
same can not be said of synthetically-generated FLAIR images. So they
used a pixel-wise neural network approach (implemented in two-dimensions) within
cGAN to improve synthetic MRI, especially for FLAIR-type
images. Separately,~\citet{daretal19} used spatial generative
adversarial networks on training sets of $\T_1$- and $\T_2$-weighted
images to predict $\T_1$  from $\T_2$ images and vice-versa. However,
this approach requires both $\T_1$- and $\T_2$-weighted training
images and is inapplicable for MRI techniques ({\em e.g.}, SPGR or
SSFP) that can not acquire them both. 
%MRI techniques. \textbf{I didn't understand the last sentence... also why will our method work?}
%\citep{gonccalvesetal18} is a new review paper - remove this paper????
In general, machine learning approaches do not work well when the
settings for the acquired scans are not in the training set. The full
potential for synthetic MRI in a clinical setting can be realized when
we are able to acquire individualized training set images and predict
synthetic images based on context and at any desired patient- or
anatomy-specific settings, and not based on some database that is an
input in an machine learning model. For example, it may be more optimal to choose
different design parameter settings when acquiring training
images for pediatric or non-cooperating patients. Further, the
individual noise characteristics of a particular MRI scanner are not
accounted for in a machine learning model. These issues are obviated in
model-based synthetic MRI which uses the physical and statistical
noise properties of the individually acquired MRI scans to synthesize
additional images at any desired design parameter settings. So here, we
provide new methods for more accurately and efficiently implementing
the framework of~\citet{maitraandriddles10}.  

The rest of our paper is as follows. Section~\ref{sec:meth} develops a
scalable  alternating expectation conditional maximization (AECM)
algorithm~\citep{mengandvandyk97} for synthetic MRI that is guaranteed
to converge and essentially matches the speed of non-regularized
methods such as LS. The key ingredients of our AECM algorithm are
a checkerboard coloring scheme~\citep{besag74,besagetal95} that allows
fast parallel block maximization over the voxel-wise
parameters and  analytically profiles out some of the GMRF parameters,
reducing the optimization over the 
remaining parameters to one in at most two
variables. An additional appealing aspect of our model-based approach
is the conceptual ease of obtaining standard error (SE) estimates of
our predictions, so we provide methods for their fast implementation
over specified regions.  
%we revisit the synthetic MRI problem, in particular, the formulation due to \citet{maitraandriddles10}, and develop a scalable EM algorithm that is guaranteed to converge and remains practically as fast as the non-regularized methods such as LS. The key ingredients of our alternating expectation conditional maximization (AECM) algorithm \citep{mengandvandyk97} are the checkerboard coloring scheme due to Besag that allows fast parallel block M-steps over the voxel-wise parameters and  analytically profiling out certain MRF parameters, reducing the M-step over the remaining parameters to an optimization problem over at most two variables. The rest of the paper is laid out as follows. In Section \ref{sec:meth} we develop the methodology and the AECM algorithm. In
Section~\ref{sec:sim} evaluates properties of our estimates, and demonstrates our methodology on a normal subject
in a clinical setting. We also investigate the selection of test sets
for optimizing predictive performance and demonstrate consistency of
our synthetic MRI predictions. A separate set of simulation
experiments evaluates estimation and prediction accuracy and
consistency for different noise levels.  
We conclude with some discussion. An online supplement with sections, figures and
tables prefixed by ``S'', is available. %at  http://dx.doi.org/10.1109/TMI.2019.2915052.
Our algorithm %Additional details are in Appendix
% \ref{sec:sim-meth}. The proposed AECM algorithm
is implemented in a C++ library \textsf{symr} (pronounced
$sim\!\cdot\!mer$) with Matlab and R~\citep{R} wrappers and uses
openMP-based parallelization for computing practicality. %and the {\em sparse} module of the {\sf Eigen} library \citep{eigenweb}. % and is wrapped as an R package \textsf{symR} and Matlab package \textsf{syMr}.  

% With Besag's checkerboard structure, the problem is parallelized, making the procedure a multicycle EM \citep{mengandrubin93}, more generally an AECM \citep{mengandvandyk97} algorithm. The optimizations for MRF parameters are also simplified with the help of profile likelihood. 
% The resulting Maximum Penalized Likelihood Estimates(MPLEs) from the
% parallelized program demonstrated excellent performance in predicting
% synthetic MR images in a clinical setting, fast, and in general,
% showed much faster convergence properties. In the next section
% \ref{sec:meth} of the paper, we would explain the methodology used in
% section \ref{sec:sim} to predict 3D synthetic images on a normal
% volunteer and a 2D phantom dataset. We investigate the selection of
% test set for optimizing predictive performance and the effect of an
% increasing number of images. Section \ref{sec:dis} discusses the
% method. Additional details are in Appendix \ref{sec:sim-meth}.
%For the sake of simplicity, we use the term `voxel' in this paper in general, which would refer to `pixel' whenever the 2D data is considered.
%We can also estimate the variance of the estimates using the information matrix from our specified model and delta method. This method is compared with parametric bootstrap for the test images which shows that for the mean vector corresponding to the different tissue types, the estimated variances are quite similar to each other. 

